Mott-moir\'e excitons

We develop a systematic theory for excitons subject to Fermi-Hubbard physics in moir\'e twisted transition metal dichalcogenides (TMDs). Specifically, we consider excitons in moir\'e systems for which the valence band is in the Mott-insulating regime. These "Mott-moir\'e excitons", which are achievable in twisted TMD heterobilayers, are bound states of a magnetic polaron in the valence band and a free electron in the conduction band. We find significantly narrower exciton bandwidths in the presence of Hubbard physics, serving as a potential experimental signature of strong correlations. We also demonstrate the high tunability of Mott-moir\'e excitons through the dependence of their binding energies, diameters, and bandwidths on the moir\'e period. Our work provides guidelines for future exploration of strongly correlated excitons in twisted TMD heterobilayers.

==> biblio_miscellaneous.tex <==


@article{Trugman1988,
  title = {Interaction of holes in a Hubbard antiferromagnet and high-temperature superconductivity},
  author = {Trugman, S. A.},
  journal = {Phys. Rev. B},
  volume = {37},
  issue = {4},
  pages = {1597--1603},
  numpages = {0},
  year = {1988},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.37.1597},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.37.1597}
}




@article{andrei2021marvels,
  title={The marvels of moir{\'e} materials},
  author={Andrei, Eva Y and Efetov, Dmitri K and Jarillo-Herrero, Pablo and MacDonald, Allan H and Mak, Kin Fai and Senthil, T and Tutuc, Emanuel and Yazdani, Ali and Young, Andrea F},
  journal={Nature Reviews Materials},
  volume={6},
  number={3},
  pages={201--206},
  year={2021},
  publisher={Nature Publishing Group}
}





@article{Wang2022light,
  title={Light-Induced Ferromagnetism in Moir$\backslash$'e Superlattices},
  author={Wang, Xi and Xiao, Chengxin and Park, Heonjoon and Zhu, Jiayi and Wang, Chong and Taniguchi, Takashi and Watanabe, Kenji and Yan, Jiaqiang and Xiao, Di and Gamelin, Daniel R and others},
  journal={arXiv preprint arXiv:2203.07161},
  year={2022}
}

@article{Shimazaki2020Strongly,
	title = {Strongly correlated electrons and hybrid excitons in a moiré heterostructure},
	volume = {580},
	issn = {1476-4687},
	url = {https://doi.org/10.1038/s41586-020-2191-2},
	doi = {10.1038/s41586-020-2191-2},
	number = {7804},
	journal = {Nature},
	author = {Shimazaki, Yuya and Schwartz, Ido and Watanabe, Kenji and Taniguchi, Takashi and Kroner, Martin and Imamoğlu, Ataç},
	month = apr,
	year = {2020},
	pages = {472--477},
}



@article{Li2021quantum,
  title={Quantum anomalous Hall effect from intertwined moir{\'e} bands},
  author={Li, Tingxin and Jiang, Shengwei and Shen, Bowen and Zhang, Yang and Li, Lizhong and Tao, Zui and Devakul, Trithep and Watanabe, Kenji and Taniguchi, Takashi and Fu, Liang and others},
  journal={Nature},
  volume={600},
  number={7890},
  pages={641--646},
  year={2021},
  publisher={Nature Publishing Group}
}


@article{Shi2021bilayer,
  title={Bilayer WSe $ \_2 $ as a natural platform for interlayer exciton condensates in the strong coupling limit},
  author={Shi, Qianhui and Shih, En-Min and Rhodes, Daniel and Kim, Bumho and Barmak, Katayun and Watanabe, Kenji and Taniguchi, Takashi and Papi{\'c}, Zlatko and Abanin, Dmitry A and Hone, James and others},
  journal={arXiv preprint arXiv:2108.10477},
  year={2021}
}

@article{Ghiotto2021quantum,
  title={Quantum criticality in twisted transition metal dichalcogenides},
  author={Ghiotto, Augusto and Shih, En-Min and Pereira, Giancarlo SSG and Rhodes, Daniel A and Kim, Bumho and Zang, Jiawei and Millis, Andrew J and Watanabe, Kenji and Taniguchi, Takashi and Hone, James C and others},
  journal={Nature},
  volume={597},
  number={7876},
  pages={345--349},
  year={2021},
  publisher={Nature Publishing Group}
}


@article{Balents2020superconductivity,
  title={Superconductivity and strong correlations in moir{\'e} flat bands},
  author={Balents, Leon and Dean, Cory R and Efetov, Dmitri K and Young, Andrea F},
  journal={Nature Physics},
  volume={16},
  number={7},
  pages={725--733},
  year={2020},
  publisher={Nature Publishing Group}
}






@misc{Su2021Massive,
      title={Massive Dirac fermions in moir\'e superlattices: a route toward correlated Chern insulators}, 
      author={Ying Su and Heqiu Li and Chuanwei Zhang and Kai Sun and Shi-Zeng Lin},
      year={2021},
      eprint={2110.02537},
      archivePrefix={arXiv},
      primaryClass={cond-mat.mes-hall}
}



@article{Anantharaman2021Exciton,
author = {Anantharaman, Surendra B. and Jo, Kiyoung and Jariwala, Deep},
title = {Exciton–Photonics: From Fundamental Science to Applications},
journal = {ACS Nano},
volume = {15},
number = {8},
pages = {12628-12654},
year = {2021},
doi = {10.1021/acsnano.1c02204},note ={PMID: 34310122},
URL = {https://doi.org/10.1021/acsnano.1c02204},
eprint = {https://doi.org/10.1021/acsnano.1c02204}
}



@article{Mueller2018Exciton,
	title = {Exciton physics and device application of two-dimensional transition metal dichalcogenide semiconductors},
	volume = {2},
	issn = {2397-7132},
	url = {https://doi.org/10.1038/s41699-018-0074-2},
	doi = {10.1038/s41699-018-0074-2},
	number = {1},
	journal = {npj 2D Materials and Applications},
	author = {Mueller, Thomas and Malic, Ermin},
	month = sep,
	year = {2018},
	pages = {29},
}


@article{Ross2014Electrically,
	title = {Electrically tunable excitonic light-emitting diodes based on monolayer {WSe2} p–n junctions},
	volume = {9},
	issn = {1748-3395},
	url = {https://doi.org/10.1038/nnano.2014.26},
	doi = {10.1038/nnano.2014.26},
	number = {4},
	journal = {Nature Nanotechnology},
	author = {Ross, Jason S. and Klement, Philip and Jones, Aaron M. and Ghimire, Nirmal J. and Yan, Jiaqiang and Mandrus, D. G. and Taniguchi, Takashi and Watanabe, Kenji and Kitamura, Kenji and Yao, Wang and Cobden, David H. and Xu, Xiaodong},
	month = apr,
	year = {2014},
	pages = {268--272},
}

@article{Konstantatos2018Current,
	title = {Current status and technological prospect of photodetectors based on two-dimensional materials},
	volume = {9},
	issn = {2041-1723},
	url = {https://doi.org/10.1038/s41467-018-07643-7},
	doi = {10.1038/s41467-018-07643-7},
	number = {1},
	journal = {Nature Communications},
	author = {Konstantatos, Gerasimos},
	month = dec,
	year = {2018},
	pages = {5266},
}


@article{Deng2010Exciton,
  title = {Exciton-polariton Bose-Einstein condensation},
  author = {Deng, Hui and Haug, Hartmut and Yamamoto, Yoshihisa},
  journal = {Rev. Mod. Phys.},
  volume = {82},
  issue = {2},
  pages = {1489--1537},
  numpages = {0},
  year = {2010},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.82.1489},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.82.1489}
}

@article{Tang2021Room,
	title = {Room temperature exciton–polariton {Bose}–{Einstein} condensation in organic single-crystal microribbon cavities},
	volume = {12},
	issn = {2041-1723},
	url = {https://doi.org/10.1038/s41467-021-23524-y},
	doi = {10.1038/s41467-021-23524-y},
	number = {1},
	journal = {Nature Communications},
	author = {Tang, Ji and Zhang, Jian and Lv, Yuanchao and Wang, Hong and Xu, Fa Feng and Zhang, Chuang and Sun, Liaoxin and Yao, Jiannian and Zhao, Yong Sheng},
	month = jun,
	year = {2021},
	pages = {3265},
}


@article{Albert2013Microcavity,
	title = {Microcavity controlled coupling of excitonic qubits},
	volume = {4},
	issn = {2041-1723},
	url = {https://doi.org/10.1038/ncomms2764},
	doi = {10.1038/ncomms2764},
	number = {1},
	journal = {Nature Communications},
	author = {Albert, F. and Sivalertporn, K. and Kasprzak, J. and Strauß, M. and Schneider, C. and Höfling, S. and Kamp, M. and Forchel, A. and Reitzenstein, S. and Muljarov, E.A. and Langbein, W.},
	month = apr,
	year = {2013},
	pages = {1747},
}

@article{ethier-majcher2014Complete,
	title = {Complete quantum control of exciton qubits bound to isoelectronic centres},
	volume = {5},
	issn = {2041-1723},
	url = {https://doi.org/10.1038/ncomms4980},
	doi = {10.1038/ncomms4980},
	number = {1},
	journal = {Nature Communications},
	author = {Éthier-Majcher, G. and St-Jean, P. and Boso, G. and Tosi, A. and Klem, J. F. and Francoeur, S.},
	month = may,
	year = {2014},
	pages = {3980},
}

@article{Wang2018Electrical,
	title = {Electrical control of charged carriers and excitons in atomically thin materials},
	volume = {13},
	issn = {1748-3395},
	url = {https://doi.org/10.1038/s41565-017-0030-x},
	doi = {10.1038/s41565-017-0030-x},
	number = {2},
	journal = {Nature Nanotechnology},
	author = {Wang, Ke and De Greve, Kristiaan and Jauregui, Luis A. and Sushko, Andrey and High, Alexander and Zhou, You and Scuri, Giovanni and Taniguchi, Takashi and Watanabe, Kenji and Lukin, Mikhail D. and Park, Hongkun and Kim, Philip},
	month = feb,
	year = {2018},
	pages = {128--132},
}




@article{Jin2019Observation,
	title = {Observation of moiré excitons in {WSe2}/{WS2} heterostructure superlattices},
	volume = {567},
	issn = {1476-4687},
	url = {https://doi.org/10.1038/s41586-019-0976-y},
	doi = {10.1038/s41586-019-0976-y},
	number = {7746},
	journal = {Nature},
	author = {Jin, Chenhao and Regan, Emma C. and Yan, Aiming and Iqbal Bakti Utama, M. and Wang, Danqing and Zhao, Sihan and Qin, Ying and Yang, Sijie and Zheng, Zhiren and Shi, Shenyang and Watanabe, Kenji and Taniguchi, Takashi and Tongay, Sefaattin and Zettl, Alex and Wang, Feng},
	month = mar,
	year = {2019},
	pages = {76--80},
}



@article{Zhang2020Twist,
	title = {Twist-angle dependence of moiré excitons in {WS2}/{MoSe2} heterobilayers},
	volume = {11},
	issn = {2041-1723},
	url = {https://doi.org/10.1038/s41467-020-19466-6},
	doi = {10.1038/s41467-020-19466-6},
	number = {1},
	journal = {Nature Communications},
	author = {Zhang, Long and Zhang, Zhe and Wu, Fengcheng and Wang, Danqing and Gogna, Rahul and Hou, Shaocong and Watanabe, Kenji and Taniguchi, Takashi and Kulkarni, Krishnamurthy and Kuo, Thomas and Forrest, Stephen R. and Deng, Hui},
	month = nov,
	year = {2020},
	pages = {5888},
}


@article{Yuan2020Twist,
	title = {Twist-angle-dependent interlayer exciton diffusion in {WS2}–{WSe2} heterobilayers},
	volume = {19},
	issn = {1476-4660},
	url = {https://doi.org/10.1038/s41563-020-0670-3},
	doi = {10.1038/s41563-020-0670-3},
	number = {6},
	journal = {Nature Materials},
	author = {Yuan, Long and Zheng, Biyuan and Kunstmann, Jens and Brumme, Thomas and Kuc, Agnieszka Beata and Ma, Chao and Deng, Shibin and Blach, Daria and Pan, Anlian and Huang, Libai},
	month = jun,
	year = {2020},
	pages = {617--623},
}

@article{Smolenski2021Signatures,
	title = {Signatures of {Wigner} crystal of electrons in a monolayer semiconductor},
	volume = {595},
	issn = {1476-4687},
	doi = {10.1038/s41586-021-03590-4},
	number = {7865},
	journal = {Nature},
	author = {Smoleński, Tomasz and Dolgirev, Pavel E. and Kuhlenkamp, Clemens and Popert, Alexander and Shimazaki, Yuya and Back, Patrick and Lu, Xiaobo and Kroner, Martin and Watanabe, Kenji and Taniguchi, Takashi and Esterlis, Ilya and Demler, Eugene and Imamoğlu, Ataç},
	month = jul,
	year = {2021},
	pages = {53--57},
}


@article{Nam1976Free,
  title = {Free-exciton energy spectrum in GaAs},
  author = {Nam, S. B. and Reynolds, D. C. and Litton, C. W. and Almassy, R. J. and Collins, T. C. and Wolfe, C. M.},
  journal = {Phys. Rev. B},
  volume = {13},
  issue = {2},
  pages = {761--767},
  numpages = {0},
  year = {1976},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.13.761},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.13.761}
}


@article{Wilson2017Determination,
author = {Neil R. Wilson  and Paul V. Nguyen  and Kyle Seyler  and Pasqual Rivera  and Alexander J. Marsden  and Zachary P. L. Laker  and Gabriel C. Constantinescu  and Viktor Kandyba  and Alexei Barinov  and Nicholas D. M. Hine  and Xiaodong Xu  and David H. Cobden },
title = {Determination of band offsets, hybridization, and exciton binding in 2D semiconductor heterostructures},
journal = {Science Advances},
volume = {3},
number = {2},
pages = {e1601832},
year = {2017},
doi = {10.1126/sciadv.1601832},
URL = {https://www.science.org/doi/abs/10.1126/sciadv.1601832},
eprint = {https://www.science.org/doi/pdf/10.1126/sciadv.1601832}
}

@article{Padhi2021Generalized,
  title = {Generalized Wigner crystallization in moir\'e materials},
  author = {Padhi, Bikash and Chitra, R. and Phillips, Philip W.},
  journal = {Phys. Rev. B},
  volume = {103},
  issue = {12},
  pages = {125146},
  numpages = {12},
  year = {2021},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.103.125146},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.103.125146}
}

@article{Mcgilly2020Visualization,
	title = {Visualization of moiré superlattices},
	volume = {15},
	issn = {1748-3395},
	url = {https://doi.org/10.1038/s41565-020-0708-3},
	doi = {10.1038/s41565-020-0708-3},
	number = {7},
	journal = {Nature Nanotechnology},
	author = {McGilly, Leo J. and Kerelsky, Alexander and Finney, Nathan R. and Shapovalov, Konstantin and Shih, En-Min and Ghiotto, Augusto and Zeng, Yihang and Moore, Samuel L. and Wu, Wenjing and Bai, Yusong and Watanabe, Kenji and Taniguchi, Takashi and Stengel, Massimiliano and Zhou, Lin and Hone, James and Zhu, Xiaoyang and Basov, Dmitri N. and Dean, Cory and Dreyer, Cyrus E. and Pasupathy, Abhay N.},
	month = jul,
	year = {2020},
	pages = {580--584},
}

@misc{Vitale2021Flat,
      title={Flat band properties of twisted transition metal dichalcogenide homo- and heterobilayers of MoS$_2$, MoSe$_2$, WS$_2$ and WSe$_2$}, 
      author={Valerio Vitale and Kemal Atalar and Arash A. Mostofi and Johannes Lischner},
      year={2021},
      eprint={2102.03259},
      archivePrefix={arXiv},
      primaryClass={cond-mat.mtrl-sci}
}

@article{ma2019dissipatively,
  title={A dissipatively stabilized Mott insulator of photons},
  author={Ma, Ruichao and Saxberg, Brendan and Owens, Clai and Leung, Nelson and Lu, Yao and Simon, Jonathan and Schuster, David I},
  journal={Nature},
  volume={566},
  number={7742},
  pages={51--57},
  year={2019},
  publisher={Nature Publishing Group}
}

@article{AlHassanieh2008Excitons,
	Author = {Al-Hassanieh, K. A. and Reboredo, F. A. and Feiguin, A. E. and Gonz\'alez, I. and Dagotto, E.},
	Journal = {Phys. Rev. Lett.},
	Month = {Apr},
	Pages = {166403},
	Title = {Excitons in the One-Dimensional Hubbard Model: A Real-Time Study},
	Volume = {100},
	Year = {2008}}




@article{Belinicher1995Hole,
	Author = {Belinicher, V. I. and Chernyshev, A. L. and Dotsenko, A. V. and Sushkov, O. P.},
	Journal = {Phys. Rev. B},
	Month = {Mar},
	Pages = {6076--6084},
	Title = {Hole-hole superconducting pairing in the t-J model induced by spin-wave exchange},
	Volume = {51},
	Year = {1995}}
    
@article{Belinicher1997Two,
	Author = {Belinicher, V. I. and Chernyshev, A. L. and Shubin, V. A.},
	Journal = {Phys. Rev. B},
	Month = {Aug},
	Pages = {3381--3393},
	Title = {Two-hole problem in the $t$-$J$ model: A canonical transformation approach},
	Volume = {56},
	Year = {1997}}
	
@article{Bloch2008Many,
	Author = {Bloch, Immanuel and Dalibard, Jean and Zwerger, Wilhelm},
	Journal = {Rev. Mod. Phys.},
	Month = {Jul},
	Pages = {885--964},
	Title = {Many-body physics with ultracold gases},
	Volume = {80},
	Year = {2008}}
	
@article{Bloch2012Quantum,
	Author = {Bloch, Immanuel and Dalibard, Jean and Nascimb{\`e}ne, Sylvain},
	Journal = {Nature Physics},
	Number = {4},
	Pages = {267--276},
	Title = {Quantum simulations with ultracold quantum gases},
	Volume = {8},
	Year = {2012}}
	
@article{Boll2016Spin,
	Author = {Boll, Martin and Hilker, Timon A. and Salomon, Guillaume and Omran, Ahmed and Nespolo, Jacopo and Pollet, Lode and Bloch, Immanuel and Gross, Christian},
	Journal = {Science},
	Month = {09},
	Number = {6305},
	Pages = {1257},
	Title = {Spin- and density-resolved microscopy of antiferromagnetic correlations in Fermi-Hubbard chains},
	Volume = {353},
	Year = {2016}}
	
@article{Brugger2006Magnon,
	Author = {Br{\"u}gger, C. and K{\"a}mpfer, F. and Pepe, M. and Wiese, U. -J.},
	Journal = {European Physical Journal B -- Condensed Matter},
	Month = {10},
	Number = {4},
	Pages = {433--437},
	Title = {Magnon-mediated binding between holes in an antiferromagnet.},
	Volume = {53},
	Year = {2006}}
	
@article{Burroughes1990Light,
	Author = {Burroughes, J. H. and Bradley, D. D. C. and Brown, A. R. and Marks, R. N. and Mackay, K. and Friend, R. H. and Burns, P. L. and Holmes, A. B.},
	Journal = {Nature},
	Number = {6293},
	Pages = {539--541},
	Title = {Light-emitting diodes based on conjugated polymers},
	Volume = {347},
	Year = {1990}}
	
@article{Byrnes2014Exciton,
	Author = {Byrnes, Tim and Kim, Na Young and Yamamoto, Yoshihisa},
	Journal = {Nature Physics},
	Month = {10},
	Pages = {803 EP -},
	Title = {Exciton--polariton condensates},
	Volume = {10},
	Year = {2014}}
	
@article{Carusotto2013Quantum,
	Author = {Carusotto, Iacopo and Ciuti, Cristiano},
	Journal = {Rev. Mod. Phys.},
	Month = {Feb},
	Pages = {299--366},
	Title = {Quantum fluids of light},
	Volume = {85},
	Year = {2013}}


@article{Eckstein2016Ultra,
	Author = {Eckstein, Martin and Werner, Philipp},
	Journal = {Scientific Reports},
	Number = {1},
	Pages = {21235},
	Title = {Ultra-fast photo-carrier relaxation in Mott insulators with short-range spin correlations},
	Volume = {6},
	Year = {2016}}
	
@article{Essler2001Excitons,
	Author = {Essler, F. H. L. and Gebhard, F. and Jeckelmann, E.},
	Journal = {Phys. Rev. B},
	Month = {Sep},
	Pages = {125119},
	Title = {Excitons in one-dimensional Mott insulators},
	Volume = {64},
	Year = {2001}}
	
@article{Esslinger2010Fermi,
	Author = {Esslinger, Tilman},
	Journal = {Annual Review of Condensed Matter Physics},
	Month = {2020/03/25},
	Number = {1},
	Pages = {129--152},
	Title = {Fermi-Hubbard Physics with Atoms in an Optical Lattice},
	Volume = {1},
	Year = {2010}}
	
@article{Gallagher1997Excitons,
	Author = {Gallagher, F. B. and Mazumdar, S.},
	Journal = {Phys. Rev. B},
	Month = {Dec},
	Pages = {15025--15039},
	Title = {Excitons and optical absorption in one-dimensional extended Hubbard models with short- and long-range interactions},
	Volume = {56},
	Year = {1997}}
	
@article{Gossling2008Mott,
	Author = {G\"ossling, A. and Schmitz, R. and Roth, H. and Haverkort, M. W. and Lorenz, T. and Mydosh, J. A. and M\"uller-Hartmann, E. and Gr\"uninger, M.},
	Journal = {Phys. Rev. B},
	Month = {Aug},
	Pages = {075122},
	Title = {Mott-Hubbard exciton in the optical conductivity of ${\text{YTiO}}_{3}$ and ${\text{SmTiO}}_{3}$},
	Volume = {78},
	Year = {2008}}
	
@article{Gregg2003Excitonic,
	Author = {Gregg, Brian A. },
	Journal = {The Journal of Physical Chemistry B},
	Month = {05},
	Number = {20},
	Pages = {4688--4698},
	Title = {Excitonic Solar Cells},
	Volume = {107},
	Year = {2003}}

@article{Gretarsson2013Crystal,
	Author = {Gretarsson, H. and Clancy, J. P. and Liu, X. and Hill, J. P. and Bozin, Emil and Singh, Yogesh and Manni, S. and Gegenwart, P. and Kim, Jungho and Said, A. H. and Casa, D. and Gog, T. and Upton, M. H. and Kim, Heung-Sik and Yu, J. and Katukuri, Vamshi M. and Hozoi, L. and van den Brink, Jeroen and Kim, Young-June},
	Journal = {Phys. Rev. Lett.},
	Month = {Feb},
	Pages = {076402},
	Title = {Crystal-Field Splitting and Correlation Effect on the Electronic Structure of ${A}_{2}{\mathrm{IrO}}_{3}$},
	Volume = {110},
	Year = {2013}}
   
@article{Hilker2017Revealing,
	Author = {Hilker, Timon A. and Salomon, Guillaume and Grusdt, Fabian and Omran, Ahmed and Boll, Martin and Demler, Eugene and Bloch, Immanuel and Gross, Christian},
	Journal = {Science},
	Month = {08},
	Number = {6350},
	Pages = {484},
	Title = {Revealing hidden antiferromagnetic correlations in doped Hubbard chains via string correlators},
	Volume = {357},
	Year = {2017}}
    

    
@article{Itkis2006Bolometric,
	Author = {Itkis, Mikhail E. and Borondics, Ferenc and Yu, Aiping and Haddon, Robert C.},
	Journal = {Science},
	Number = {5772},
	Pages = {413--416},
	Title = {Bolometric Infrared Photoresponse of Suspended Single-Walled Carbon Nanotube Films},
	Volume = {312},
	Year = {2006}}
	
@article{Kane1989Motion,
	Author = {Kane, C. L. and Lee, P. A. and Read, N.},
	Journal = {Phys. Rev. B},
	Month = {Apr},
	Pages = {6880--6897},
	Title = {Motion of a single hole in a quantum antiferromagnet},
	Volume = {39},
	Year = {1989}}
	
@article{Kasprzak2006Bose,
	Author = {Kasprzak, J. and Richard, M. and Kundermann, S. and Baas, A. and Jeambrun, P. and Keeling, J. M. J. and Marchetti, F. M. and Szyma{\'n}ska, M. H. and Andr{\'e}, R. and Staehli, J. L. and Savona, V. and Littlewood, P. B. and Deveaud, B. and Dang, Le Si},
	Journal = {Nature},
	Number = {7110},
	Pages = {409--414},
	Title = {Bose--Einstein condensation of exciton polaritons},
	Volume = {443},
	Year = {2006}}
	
@article{Keeling2007Collective,
	Author = {J Keeling and F M Marchetti and M H Szyma{\'{n}}ska and P B Littlewood},
	Journal = {Semiconductor Science and Technology},
	Month = {apr},
	Number = {5},
	Pages = {R1--R26},
	Title = {Collective coherence in planar semiconductor microcavities},
	Volume = {22},
	Year = 2007}
	
@article{Kim2014Excitonic,
	Author = {Kim, Jungho and Daghofer, M. and Said, A. H. and Gog, T. and van den Brink, J. and Khaliullin, G. and Kim, B. J.},
	Journal = {Nature Communications},
	Number = {1},
	Pages = {4453},
	Title = {Excitonic quasiparticles in a spin--orbit Mott insulator},
	Volume = {5},
	Year = {2014}}
	


	
@article{Kuchiev1993Large,
	Author = {Kuchiev, M. Yu. and Sushkov, O. P.},
	Journal = {Physica C: Superconductivity},
	Number = {1},
	Pages = {197--207},
	Title = {Large-size two-hole bound states in the t-J model},
	Volume = {218},
	Year = {1993}}

	
@article{Lee2006Doping,
	Author = {Lee, Patrick A. and Nagaosa, Naoto and Wen, Xiao-Gang},
	Journal = {Rev. Mod. Phys.},
	Month = {Jan},
	Pages = {17--85},
	Title = {Doping a Mott insulator: Physics of high-temperature superconductivity},
	Volume = {78},
	Year = {2006}}
	
@article{Li1989Spin,
	Author = {Li, T. and W\"olfle, P. and Hirschfeld, P. J.},
	Journal = {Phys. Rev. B},
	Month = {Oct},
	Pages = {6817--6821},
	Title = {Spin-rotation-invariant slave-boson approach to the Hubbard model},
	Volume = {40},
	Year = {1989}}

@article{MacDonald1988Expansion,
	Author = {MacDonald, A. H. and Girvin, S. M. and Yoshioka, D.},
	Journal = {Phys. Rev. B},
	Month = {Jun},
	Pages = {9753--9756},
	Title = {$\frac{t}{U}$ expansion for the Hubbard model},
	Volume = {37},
	Year = {1988}}
	
@article{Matsueda2005Excitonic,
	Author = {Matsueda, H. and Tohyama, T. and Maekawa, S.},
	Journal = {Phys. Rev. B},
	Month = {Apr},
	Pages = {153106},
	Title = {Excitonic effect on the optical response in the one-dimensional two-band Hubbard model},
	Volume = {71},
	Year = {2005}}

@article{Nakanishi1969General,
	Author = {Nakanishi, Noboru},
	Journal = {Progress of Theoretical Physics Supplement},
	Month = {01},
	Pages = {1-81},
	Title = {A General Survey of the Theory of the Bethe-Salpeter Equation},
	Volume = {43},
	Year = {1969}}
	
@article{Novelli2012Ultrafast,
	Author = {Novelli, Fabio and Fausti, Daniele and Reul, Julia and Cilento, Federico and van Loosdrecht, Paul H. M. and Nugroho, Agung A. and Palstra, Thomas T. M. and Gr\"uninger, Markus and Parmigiani, Fulvio},
	Journal = {Phys. Rev. B},
	Month = {Oct},
	Pages = {165135},
	Title = {Ultrafast optical spectroscopy of the lowest energy excitations in the Mott insulator compound YVO${}_{3}$: Evidence for Hubbard-type excitons},
	Volume = {86},
	Year = {2012}}
	
@article{Ogawa1975Gutzwiller,
	Author = {Ogawa, Tohru and Kanda, Kunihiko and Matsubara, Takeo},
	Journal = {Progress of Theoretical Physics},
	Month = {3/15/2020},
	Number = {3},
	Pages = {614--633},
	Title = {Gutzwiller Approximation for Antiferromagnetism in Hubbard Model *)},
	Volume = {53},
	Year = {1975}}
	
@article{Ono2005Direct,
	Author = {Ono, M. and Kishida, H. and Okamoto, H.},
	Journal = {Phys. Rev. Lett.},
	Month = {Aug},
	Pages = {087401},
	Title = {Direct Observation of Excitons and a Continuum of One-Dimensional Mott Insulators: A Reflection-Type Third-Harmonic-Generation Study of Ni-Halogen Chain Compounds},
	Volume = {95},
	Year = {2005}}
	
@article{Parsons2016Site,
	Author = {Parsons, Maxwell F. and Mazurenko, Anton and Chiu, Christie S. and Ji, Geoffrey and Greif, Daniel and Greiner, Markus},
	Journal = {Science},
	Month = {09},
	Number = {6305},
	Pages = {1253},
	Title = {Site-resolved measurement of the spin-correlation function in the Fermi-Hubbard model},
	Volume = {353},
	Year = {2016}}
	
@book{Plakida2010,
    Author = {Plakida, N.},
    Publisher = {Springer Berlin Heidelberg},
    Title = {High-Temperature Cuprate Superconductors: Experiment, Theory, and Applications},
    Year = {2010}}
	
@article{Plumhof2014Room,
	Author = {Plumhof, Johannes D. and St{\"o}ferle, Thilo and Mai, Lijian and Scherf, Ullrich and Mahrt, Rainer F.},
	Journal = {Nature Materials},
	Number = {3},
	Pages = {247--252},
	Title = {Room-temperature Bose--Einstein condensation of cavity exciton--polaritons in a polymer},
	Volume = {13},
	Year = {2014}}
	
@article{Salomon2019Direct,
	Author = {Salomon, Guillaume and Koepsell, Joannis and Vijayan, Jayadev and Hilker, Timon A. and Nespolo, Jacopo and Pollet, Lode and Bloch, Immanuel and Gross, Christian},
	Journal = {Nature},
	Number = {7737},
	Pages = {56--60},
	Title = {Direct observation of incommensurate magnetism in Hubbard chains},
	Volume = {565},
	Year = {2019}}

@article{SchmittRink1988Spectral,
	Author = {Schmitt-Rink, S. and Varma, C. M. and Ruckenstein, A. E.},
	Journal = {Phys. Rev. Lett.},
	Month = {Jun},
	Pages = {2793--2796},
	Title = {Spectral Function of Holes in a Quantum Antiferromagnet},
	Volume = {60},
	Year = {1988}}
	
@article{Schneider2008Metallic,
	Author = {Schneider, U. and Hackerm{\"u}ller, L. and Will, S. and Best, Th. and Bloch, I. and Costi, T. A. and Helmes, R. W. and Rasch, D. and Rosch, A.},
	Journal = {Science},
	Number = {5907},
	Pages = {1520--1525},
	Title = {Metallic and Insulating Phases of Repulsively Interacting Fermions in a 3D Optical Lattice},
	Volume = {322},
	Year = {2008}}
	
@article{Shraiman1989Mean,
	Author = {Shraiman, Boris I. and Siggia, Eric D.},
	Journal = {Phys. Rev. B},
	Month = {Nov},
	Pages = {9162--9166},
	Title = {Mean-field theory for vacancies in a quantum antiferromagnet},
	Volume = {40},
	Year = {1989}}
	

@article{Vijayan2020Time,
	Author = {Vijayan, Jayadev and Sompet, Pimonpan and Salomon, Guillaume and Koepsell, Joannis and Hirthe, Sarah and Bohrdt, Annabelle and Grusdt, Fabian and Bloch, Immanuel and Gross, Christian},
	Journal = {Science},
	Month = {01},
	Number = {6474},
	Pages = {186},
	Title = {Time-resolved observation of spin-charge deconfinement in fermionic Hubbard chains},
	Volume = {367},
	Year = {2020}}

@article{VonSzczepanski1990Single,
	Author = {von Szczepanski, K. J. and Horsch, P. and Stephan, W. and Ziegler, M.},
	Journal = {Phys. Rev. B},
	Month = {Feb},
	Pages = {2017--2029},
	Title = {Single-particle excitations in a quantum antiferromagnet},
	Volume = {41},
	Year = {1990}}
	
@article{Wrobel2002Excitons,
	Author = {Wr\'obel, P. and Eder, R.},
	Journal = {Phys. Rev. B},
	Month = {Jul},
	Pages = {035111},
	Title = {Excitons in Mott insulators},
	Volume = {66},
	Year = {2002}}
	
	
	
	


@article{Jin2018Imaging,
author = {Chenhao Jin  and Jonghwan Kim  and M. Iqbal Bakti Utama  and Emma C. Regan  and Hans Kleemann  and Hui Cai  and Yuxia Shen  and Matthew James Shinner  and Arjun Sengupta  and Kenji Watanabe  and Takashi Taniguchi  and Sefaattin Tongay  and Alex Zettl  and Feng Wang },
title = {Imaging of pure spin-valley diffusion current in WS<sub>2</sub>-WSe<sub>2</sub> heterostructures},
journal = {Science},
volume = {360},
number = {6391},
pages = {893-896},
year = {2018},
doi = {10.1126/science.aao3503}
}



@article{Shimazaki2021Optical,
  title = {Optical Signatures of Periodic Charge Distribution in a Mott-like Correlated Insulator State},
  author = {Shimazaki, Yuya and Kuhlenkamp, Clemens and Schwartz, Ido and Smole\ifmmode \acute{n}\else \'{n}\fi{}ski, Tomasz and Watanabe, Kenji and Taniguchi, Takashi and Kroner, Martin and Schmidt, Richard and Knap, Michael and Imamo\ifmmode \breve{g}\else \u{g}\fi{}lu, Ata\ifmmode \mbox{\c{c}}\else \c{c}\fi{}},
  journal = {Phys. Rev. X},
  volume = {11},
  issue = {2},
  pages = {021027},
  numpages = {10},
  year = {2021},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevX.11.021027}
}



@article{
Gross2017Quantum,
author = {Christian Gross  and Immanuel Bloch },
title = {Quantum simulations with ultracold atoms in optical lattices},
journal = {Science},
volume = {357},
number = {6355},
pages = {995-1001},
year = {2017},
doi = {10.1126/science.aal3837},
URL = {https://www.science.org/doi/abs/10.1126/science.aal3837},
eprint = {https://www.science.org/doi/pdf/10.1126/science.aal3837}}


@article{Hartke2020Doublon,
  title = {Doublon-Hole Correlations and Fluctuation Thermometry in a Fermi-Hubbard Gas},
  author = {Hartke, Thomas and Oreg, Botond and Jia, Ningyuan and Zwierlein, Martin},
  journal = {Phys. Rev. Lett.},
  volume = {125},
  issue = {11},
  pages = {113601},
  numpages = {6},
  year = {2020},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.125.113601},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.125.113601}
}



@article{
Cheuk2016Observation,
author = {Lawrence W. Cheuk  and Matthew A. Nichols  and Katherine R. Lawrence  and Melih Okan  and Hao Zhang  and Ehsan Khatami  and Nandini Trivedi  and Thereza Paiva  and Marcos Rigol  and Martin W. Zwierlein },
title = {Observation of spatial charge and spin correlations in the 2D Fermi-Hubbard model},
journal = {Science},
volume = {353},
number = {6305},
pages = {1260-1264},
year = {2016},
doi = {10.1126/science.aag3349},
URL = {https://www.science.org/doi/abs/10.1126/science.aag3349},
eprint = {https://www.science.org/doi/pdf/10.1126/science.aag3349}}


@article{
Brown2017Spin,
author = {Peter T. Brown  and Debayan Mitra  and Elmer Guardado-Sanchez  and Peter Schauß  and Stanimir S. Kondov  and Ehsan Khatami  and Thereza Paiva  and Nandini Trivedi  and David A. Huse  and Waseem S. Bakr },
title = {Spin-imbalance in a 2D Fermi-Hubbard system},
journal = {Science},
volume = {357},
number = {6358},
pages = {1385-1388},
year = {2017},
doi = {10.1126/science.aam7838},
URL = {https://www.science.org/doi/abs/10.1126/science.aam7838},
eprint = {https://www.science.org/doi/pdf/10.1126/science.aam7838}}



@article{
Brown2019Bad,
author = {Peter T. Brown  and Debayan Mitra  and Elmer Guardado-Sanchez  and Reza Nourafkan  and Alexis Reymbaut  and Charles-David Hébert  and Simon Bergeron  and A.-M. S. Tremblay  and Jure Kokalj  and David A. Huse  and Peter Schauß  and Waseem S. Bakr },
title = {Bad metallic transport in a cold atom Fermi-Hubbard system},
journal = {Science},
volume = {363},
number = {6425},
pages = {379-382},
year = {2019},
doi = {10.1126/science.aat4134},
URL = {https://www.science.org/doi/abs/10.1126/science.aat4134},
eprint = {https://www.science.org/doi/pdf/10.1126/science.aat4134}}




==> section_A8.tex <==
\section{Incompressibility for the Hubbard model}
\label{Appendix_Incompressibility_Hubbard model}

In this section, we calculate the incompressibility of Hubbard model with a varying chemical potential $\mu$ as an estimation for the incompressible state due to charge order in the valence moir\'e band.
We follow the approach of high temperature expansion outlined in Ref.~\cite{Hingorani2022Onset}, in the limit $\beta t\ll 1$, where $\beta$ is the inverse temperature, such that the effect of hopping, and hence the spin Heisenberg exchange, is washed out by temperature.
To start with, the grand partition function $Z$ is written as:
\begin{equation}
\label{eq:Grand_partition_function_Hubbard}
Z=Tr\exp\left[-\beta\hat{H}_{hub}+\mu\sum_{i\tau}\hat{v}_{i\tau}^\dagger\hat{v}_{i\tau}\right]
,
\end{equation}
where $\hat{H}_{hub}$ is given by Eq.~\eqref{eq:Hubbard_model_def}.
Now the high temperature expansion described in Ref.~\cite{Hingorani2022Onset} with $\beta t\ll 1$ tells that one can write $\ln Z$ in terms of power series in $\beta t$.
For our purpose, it is sufficient to keep only the zeroth order $N^{-1}\ln Z\simeq z_0$, where $z_0$ is the single-site grand partition function evaluated from taking $t=0$ for Eq.~\eqref{eq:Grand_partition_function_Hubbard}.
Explicitly, one has:
\begin{equation}
z_0=1+2\zeta+\zeta^2w
,
\end{equation}
where $\zeta=e^{\beta\mu}$ and $w=e^{-\beta U}$.
The valence moir\'e band charge density $\rho_v$ and the associated incompressibility $\kappa_c^{-1}$ follows directly as:
\begin{equation}
\rho_v
=
\zeta\frac{\partial}{\partial\zeta}\ln z_0
=
\frac{2\zeta(1+\zeta w)}{1+2\zeta+\zeta^2w}
\end{equation}
\begin{equation}
\label{eq:incompressibility_Hubbard}
\kappa_c
=
\beta\zeta\frac{\partial\rho_v}{\partial\zeta}
=
\frac{2\beta\zeta(1+2w\zeta+w\zeta^2)}{(1+2\zeta+\zeta^2w)^2}
.
\end{equation}
The minimum of $\kappa_c(\zeta)$ lies at $\zeta=w^{-1/2}$.
From numerics, one could see that $\mu=U/2$, or $\zeta=w^{-1/2}$, gives the local minimum $\kappa_c=\beta\sqrt{w}/(1+\sqrt{w})$.
Hence, the local maximum of incompressibility at $\mu=U/2$ is:
\begin{equation}
\label{eq:incompressibility_peak}
\kappa_c^{-1}\big|_{\mu=\frac{U}{2}}=\frac{1+e^{\frac{\beta U}{2}}}{\beta}
\end{equation}
To make further analysis, we assume that $w\ll1$, meaning low temperature compared to $U$.
In this limit, one can see that the second term is dominating; hence the peak value of incompressibility scales as $\kappa_c^{-1}\big|_{\mu=\frac{U}{2}}\simeq\beta^{-1}e^{\frac{\beta U}{2}}$.
Also, in the same limit, one can solve analytically for the half-width of such incompressibility peaked near $\mu=U/2$, which is:
\begin{equation}
\Delta_{\frac{1}{2}}\mu
\simeq
\frac{1}{\beta}
\left[
\ln\left(\frac{2+\sqrt{3}}{2-\sqrt{3}}\right)
+
\frac{10\sqrt{w}}{\sqrt{3}}
\right]
.
\end{equation}
Hence, one sees that in the limit $\beta U\gg 1$, this half-width scales as temperature.
A last comment on this analysis is that the regime for temperature therein is $U\gg T\gg t$, which is totally different from that of the regime discussed in the main text $T\ll J$.
Hence, the spin physics in the analysis here is completely ignored.
The plot between incompressibility and filling fraction in shown in Fig.~\ref{fig_incompressibility}

\begin{figure}[t]
\centering
\includegraphics[width=1.0\columnwidth]{fig_incompressibility.pdf}
\caption{Incompressibility of the Hubbard model according to Eq.~\eqref{eq:incompressibility_Hubbard}. $\kappa_{c1}$ denotes the compressibility evaluated at filling fraction $1$, which is at $\mu=U/2$, and is provided by Eq.~\eqref{eq:incompressibility_peak}. $\rho_v$ is the density of electron in the valence moir\'e band, or equivalently the filling fraction.}
\label{fig_incompressibility}
\end{figure}








==> section_A_U0_attraction.tex <==
\section{Correction on on-site Coulomb attraction} 
\label{Appendix_U0}


\begin{figure}[t]
\centering
\includegraphics[width=1.0\columnwidth]{fig_on_site_Coulomb.pdf}
\caption{On-site Coulomb energy $V_0$ based on Eq.~\eqref{eq:Coulomb_no_gate_screening} (solid triangle) and $V_0=U$ (unfilled triangles).
$V_1$ is also included in the figure.
The dielectric constant is set as $\epsilon_r=10$.
}
\label{fig_on_site_Coulomb}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=1.0\columnwidth]{fig_exciton_properties_U.pdf}
\caption{Properties of Mott-moir\'e excitons at $m=0.48$ as functions of moir\'e period $a_M$ comparing $V_0$ based on Eq.~\eqref{eq:Coulomb_no_gate_screening} (solid triangle) and $V_0=U$ (unfilled triangles).
The dielectric constant for Coulomb binding is set as $\epsilon_r=10$.
System for numerical calculation consists of $N=3\times24^2$ moir\'e sites.
(a) The binding energy of the lowest internal state $E_{0,\bm{Q}}^B$ evaluated at $\bm{Q}=\bm{\kappa}$, which is the momenta giving the largest binding for both Mott-moir\'e and moir\'e excitons, scaled with $V_0$. 
(b) The average diameter of excitons, evaluated using the wavefunctions at respectively total momenta $\bm{Q}=\bm{\kappa}$. 
(c) The exciton band-widths $W_X$ for Mott-moir\'e, scaled with $E_s=t^2/(V_0-V_1)$. 
The values for $t$ and $J$ (as a function of the moir\'e period $a_M$) from Ref.~\cite{Wu2018Hubbard} for WSe\textsubscript{2} on top of MoSe\textsubscript{2}, which are included in Fig.~\ref{fig_Jandt}, are used. 
}
\label{fig_exciton_properties_U}
\end{figure}

\yz{(YZ: Is this appendix important to anything discussed in the main text? I am a bit worried about the analysis here. Microscopically, the short-range Coulomb interaction can be computed. The form we used in the main text is the long-range component of Coulomb interaction. I think it is good to state what we generally expect, but I don't think we can say much about the actual short-range interaction without doing complicated microscopic calculations.)}

As mentioned in Section~\ref{sec:formalism}, the expression of Coulomb attraction between electron and holon Eq.~\eqref{eq:Coulomb_no_gate_screening} does not include the effect of spatial spread of Wannier orbitals of electrons and holons, which results in an overestimation of Coulomb attraction.
To justify that Eq.~\eqref{eq:Coulomb_no_gate_screening} is qualitatively correct, we present the calculation in which the on-site Coulomb interaction between electron and holon is approximated by $-U$, which is minus the Hubbard repulsion.
This is valid as we assume that the size of Wannier orbitals of the hole and electron are roughly the same.
Comparison between the energy scales $V_0$ and $U$ are shown in Fig.~\ref{fig_on_site_Coulomb}.
We see that $V_0$ overestimates the on-site Coulomb attraction.

Keeping all off-site Coulomb interactions being inversely proportional to the electron-holon separation, we have:
\begin{equation}
\label{eq:Coulomb__corrected}
V(q)
=
\frac{2\pi e^2}{\epsilon_r}\frac{1}{q}
-
\frac{U-V_0}{N}
.
\end{equation}
Comparison between the results based on this expression and the ones from Eq.~\eqref{eq:Coulomb_no_gate_screening} is shown in Fig.~\ref{fig_exciton_properties_U}.
We see that the qualitative trends for the two different on-site Coulomb attractions $V_0$ and $U$ are the same. 
Also, we see that the exciton size with $U$ is larger than that with $V_0$, which is a direct consequence of $U<V_0$.





















